Benefits of over-parameterization with EM

Expectation Maximization (EM) is among the most popular algorithms for maximum likelihood estimation, but it is generally only guaranteed to find its stationary points of the log-likelihood objective. The goal of this article is to present theoretical and empirical evidence that over-parameterization can help EM avoid spurious local optima in the log-likelihood. We consider the problem of estimating the mean vectors of a Gaussian mixture model in a scenario where the mixing weights are known. Our study shows that the global behavior of EM, when one uses an over-parameterized model in which the mixing weights are treated as unknown, is better than that when one uses the (correct) model with the mixing weights fixed to the known values. For symmetric Gaussians mixtures with two components, we prove that introducing the (statistically redundant) weight parameters enables EM to find the global maximizer of the log-likelihood starting from almost any initial mean parameters, whereas EM without this over-parameterization may very often fail. For other Gaussian mixtures, we provide empirical evidence that shows similar behavior. Our results corroborate the value of over-parameterization in solving non-convex optimization problems, previously observed in other domains.

==> proof.tex <==


%\section{Analysis of known weights case}\label{sec:knownweights}
%\begin{lemma}\label{lem:Hequalw}
%$H(\theta;\theta^*,\frac{1}{2})$ is concave in $\theta\geq 0$ and convex in $\theta\leq 0$. Further, $\theta \in \{0,-\theta^*,\theta^*\}$ are the only three fixed points  and only $\theta^*$ and $-\theta^*$ are the stable fixed points.
%\end{lemma}
\subsection{Roadmap of the proof for Theorem \ref{thm:main}}\label{sec:mainproof}

Our first lemma that will be proved in Section \ref{sec:proofinitialarea} of the supplementary file confirms that if $\dotp{\vpt{0},\vtheta^*}>0$, then $\dotp{\vpt{t},\vtheta^*}>0$ for every $t$ and $\pw{t}_1\in (0.5,1)$. In other words, the estimates of the population-${\rm EM}_2$ remain in the correct hyper plane and the weight moves in the right direction too. 

\begin{lemma} \label{lem:initialarea} 
If $\dotp{\vpt{0},\vtheta^*}>0$, we have $\dotp{\vpt{t},\vtheta^*}>0, \pw{t}_1\in (0.5,1)$ for all $t\geq 1$. Otherwise, if $\dotp{\vpt{0},\vtheta^*}<0$, we have $\dotp{\vpt{t},\vtheta^*}<0, \pw{t}_1\in (0,0.5)$ for all $t\geq 1$.
\end{lemma}

Hence, by combining \eqref{eq:sign} and Lemma \ref{lem:initialarea}, we can safely assume that $\dotp{\vpt{t},\vtheta^*}>0$ and $\pw{t}_1\in (0.5,1)$ for all $t\geq 1$. Let $d$ be the dimension of $\vtheta^*$. We will show that the proof for the case $d>1$ can be reduced to the proof of $d=1$. This reduction is done by proving that the angle between the two vectors $\vpt{t}$ and $\vtheta^*$ is a decreasing function of $t$ and converges to $0$ (See Section \ref{sec:reduceto1} of the supplementary file). Hence, in the rest of this section we focus on the proof of Theorem \ref{thm:main} for $d=1$. Let $g_{\theta}(\theta,w_1)$ and $g_w(\theta,w_1)$ be the shorthand for the two update functions $G_{\theta}$ and $G_w$ defined in \eqref{eq:update2w} and \eqref{eq:update2theta} for a fixed $(\theta^*,w^*_1)$. To prove that $\{(\pt{t},\pw{t})\}$ converges to the fixed point $(\theta_{\star},w_{\star})$, we need the following pieces:
\begin{itemize}
\item[C.1] There exists a set $S=(a_{\theta},b_{\theta})\times (a_w,b_w)\in \bbR^2$, where $a_{\theta},b_{\theta}\in \bbR\bigcup \{\pm\infty\}$ and $a_w,b_w\in \bbR$, such that $S$ contains point $(\theta_{\star},w_{\star})$ and point $(g_{\theta}(\theta,w_1),g_w(\theta,w_1))\in S$ for all $(\theta,w_1)\in S$. Further, $g_{\theta}(\theta,w_1)$ is a non-decreasing function of $\theta$ for a given $w_1\in(a_w,b_w)$ and $g_{w}(\theta,w_1)$ is a non-decreasing function of $w$ for a given $\theta\in(a_{\theta},b_{\theta})$,
\item[C.2] There exists a ``reference curve'' function $r: [a_w,b_w] \rightarrow [a_{\theta},b_{\theta}]$ defined on $\bar{S}$, the closure of $S$, such that
\begin{itemize}
\item[C.2a] $r$ is continuous, decreasing and it passes through point $(\theta_{\star},w_{\star})$, i.e., $r(w_{\star})=\theta_{\star}.$ %Further, we have
%$\lim_{w\rightarrow a_w} r(w)=b_{\theta}$ and $r(b_w)>a_{\theta}$.
\item[C.2b] 
Given $\theta \in (a_{\theta},b_{\theta})$, function $w \mapsto g_w(\theta,w)$ has a stable fixed point in $[a_w,b_w]$. Further, any stable fixed point $w_s$ in $[a_w,b_w]$ or fixed point $w_s$ in $(a_w,b_w)$ satisfies the following:
\begin{itemize}
\item If $\theta<\theta_{\star}$ and $\theta\geq r(b_w)$, then $r^{-1}(\theta)>w_s>w_{\star}$. 
\item If $\theta=\theta_{\star}$, then $r^{-1}(\theta)=w_s=w_{\star}$.  
\item If $\theta>\theta_{\star}$ and $\theta\leq r(a_w)$, then $r^{-1}(\theta)<w_s<w_{\star}$.  
\end{itemize}  
\item[C.2c] Given $w\in [a_w,b_w]$, function $\theta \mapsto g_{\theta}(\theta,w)$ has a stable fixed point in $[a_{\theta},b_{\theta}]$. Further, any stable fixed point $\theta_s$ in $[a_{\theta},b_{\theta}]$ or fixed point $\theta_s$ in $(a_{\theta},b_{\theta})$ satisfies the following:
\begin{itemize}
\item If $w_1<w_{\star}$, then $r(w)> \theta_s>\theta_{\star}$.  
\item If $w_1=w_{\star}$, then $r(w)=\theta_s=\theta_{\star}$.  
\item If $w_1>w_{\star}$, then $r(w)< \theta_s<\theta_{\star}$.  
\end{itemize} 
%\item[C.5] $(\theta_{\star},w_{\star})$ is the only one solution of
%\begin{eqnarray}
%\theta &=&f(\theta,w)\n\\
%w &=&g(\theta,w).\n
%\end{eqnarray} 
\end{itemize}
\end{itemize}
We explain C.1 and C.2 in Figure \ref{fig:convergef}. Heuristically, we expect $(\theta^*,w^*_1)$ to be the only fixed point of the mapping $(\theta, w)\mapsto (g_{\theta}(\theta,w), g_{w}(\theta,w))$, and that $(\pt{t},\pw{t})$ move toward this fixed point. Hence, we can prove the convergence of the iterates by showing certain geometric relations between the fixed point curves of the two functions. Hence, C.1 helps us to bound the iterates on the area that such nice geometric relations exist, and the reference curve $r$ and C.2 are the tools to help us mathematically characterizing the geometric relations shown in the figure. Indeed, the next lemma implies that $C.1$ and $C.2$ are sufficient to show the convergence to the right point $(\theta_{\star},w_{\star})$:
\begin{lemma}[Supplementary \ref{sec:proofconverge}]\label{lem:converge}
Suppose continuous functions $g_{\theta}(\theta,w),g_w(\theta,w)$ satisfy $C.1$ and $C.2$,  then there exists a continuous mapping $m:\bar{S}\rightarrow [0,\infty)$ such that $(\theta_{\star},w_{\star})$ is the only solution for $m(\theta,w)=0$ on $\bar{S}$, the closure of $S$\footnote{The closure of $S$ is considered $[a_{\theta},b_{\theta}]\times [a_w,b_w]$ even when $a_{\theta},b_{\theta}\in \{\pm\infty\}$.}. Further, if we initialize $(\pt{0},\pw{0})$ in $S$, the sequence $\{(\pt{t},\pw{t})\}_{t\geq 0}$ defined by
\begin{eqnarray}
\pt{t+1}&=&g_{\theta}(\pt{t},\pw{t}), \kand  \pw{t+1}\= g_w(\pt{t},\pw{t}),\n
\end{eqnarray}  
satisfies that $m(\pt{t},\pw{t})\downarrow 0$, and therefore $(\pt{t},\pw{t})$ converges to $(\theta_{\star},w_{\star})$.
\end{lemma}  

In our problem, we set $a_w=0.5, b_w=1, a_{\theta}=0,b_{\theta}=\infty$ and $(\theta_{\star},w_{\star})=(\theta^*,w^*_1)$. Then according to Lemma \ref{lem:initialarea} and monotonic property of $g_{\theta}$ and $g_w$, C.1 is satisfied, and therefore we just need to show C.2.  First, let us define the reference curve $r$ by
\begin{eqnarray}
r(w_1): = \frac{w^*_1-w^*_2}{w_1-w_2}\theta^* \= \frac{2w^*_1-1}{2w_1-1}\theta^*, \quad \quad \forall w_1\in (0.5,1],w_2=1-w_1.\label{eq:r}
\end{eqnarray}
Hence, C.2a clearly holds. To show C.2b, notably, the weights update function $g_w(\theta,w)$ has a nice property stronger than the requirement of C.2b. In fact we can show that for any fixed $\theta>0$, function $w_1 \mapsto g_w(\theta, w_1)$ has at most one other fixed point besides $w_1=0$ and $w_1=1$, and most importantly, it has only one unique stable fixed point, i.e.,
\begin{lemma}[Supplementary \ref{sec:proofshapeg}] \label{lem:shapeg}
For all $\theta>0$, there are at most three fixed points for $g_w(\theta,w_1)$ with respect to $w_1$. Further, there exists an unique stable fixed point $F_w(\theta)\in (0,1]$, i.e., (i) $F_w(\theta)= g_w(\theta,F_w(\theta))$ and (ii) for all $w_1\in (0,1)$, we have
\begin{eqnarray}
g_w(\theta,w_1)\lessgtr w_1 \quad \text{is equivalent to} \quad w_1\gtrless F_w(\theta).\label{eq:shapeofg}
%g_w(\theta,w_1)>w_1\quad \text{is equivalent to} \quad w_1<F_w(\theta).\label{eq:shapeofg}
\end{eqnarray}
\end{lemma}
We explain Lemma \ref{lem:shapeg} in Figure \ref{fig:Model1H}. Note that, in the figure, we observe that $g_w$ is an increasing function with $g_w(\theta,0)=0$ and $g_w(\theta,1)=1$. Further, it is either a concave function or concave-convex function (first concave and then convex). Hence, we know if $\partial g_{w}(\theta,w_1)/\partial w_1|_{w_1=1}$ is at most $1$, the only stable fixed point is $w_1=1$, else if the derivative is larger than 1, there exists only one fixed point in (0,1) and it is the only stable fixed point. The complete proof for C.2b is shown in supplementary \ref{sec:proofc2bfirst}.
%\subsubsection{Analysis of the fixed points for $\boldsymbol{g_w(\theta,w_1)}$}\label{sec:anag_w}
%The rest of the proof is very technical and is shown in supplementary \ref{sec:proofc2b2b}. 

The finial step to apply Lemma \ref{lem:converge} is to prove C2.c. However, $(\theta,w_1)=((2w^*_1-1)\theta^*,1)$ is a point on the reference curve $r$ and $\theta=(2w^*_1-1)\theta^*$ is a stable fixed point for $g_{\theta}(\theta,1)$. This violates C.2c. To adjust this issue, since we can characterize the shape and the number of fixed points for $g_w$, by typical uniform continuity arguments, we can find $\delta,\epsilon>0$ such that the adjusted reference curve $r_{adj}(w):=r(w)-\epsilon\cdot \max(0,w-1+\delta)$ satisfies C.2a and C.2b. Then we can prove that the adjusted reference curve $r_{adj}(w)$ satisfies C2.c as well in supplementary \ref{sec:proofc2c}.

\begin{figure}
\begin{center}
\includegraphics[width=0.65\textwidth]{vic2.pdf}
\end{center}
\caption{The functions $g_{\theta}$ and $g_w$ are shown with red and blue lines respectively. The green point at the intersections of the three curves is the correct convergence point $(\theta_{\star},w_{\star})$. The black dotted curve shows the reference curve $r$. The cross points $\times$ are the possible initializations and the plus points $+$ are the corresponding positions after the first iteration. By the geometric relations between the three curves, the iterations have to converge to $(\theta_{\star},w_{\star})$}
\label{fig:convergef}
\end{figure}



%\subsection{Analysis of $g_{w}(w,\theta)$ and its fixed points }
%In this section, we will first show that $g_w(w,\theta)$ has a nice shape, i.e,
%\begin{lemma}\label{lem:gshape}
%For any given $\theta\neq 0$, we have $g_w(w,\theta)$ should satisfy the following case 1 or case 3 if $\theta>0$, otherwise, $g_w(w,\theta)$ can should satisfy the following case 2 or case 3.
%\begin{itemize}
%\item Case 1: $g_w(w,\theta)$ is strictly concave with respect to $w$. 
%\item Case 2: $g_w(w,\theta)$ is strictly convex with respect to $w$.
%\item Case 3: $g_w(w,\theta)$ is first strictly concave then strictly convex with respect to $w$.
%\end{itemize}
%\end{lemma}
%~\\
%Then, since $g_w(1,\theta)=1$ and $g_w(0,\theta)=0$, we know that 
%\begin{itemize}
%\item If $g_w(w,\theta)$ satisfies case 1, we have $w=1$ is the only stable fixed point.
%\item If $g_w(w,\theta)$ satisfies case 2, we have $w=0$ is the only stable fixed point.
%\item If $g_w(w,\theta)$ satisfies case 3, there exist one fixed point between $(0,1)$ and it is the only stable fixed point.
%\end{itemize}
%Further, 

%
%by continuity of the function, there exists $\delta>0$ such that
%$$H(\theta_0;\theta^*,w_1)<\theta_0, \quad \quad \forall w_1\in [\frac{1}{2},\frac{1}{2}+\delta].$$
%Combine with \eqref{eq:H_eq1} and use continuity of the function again, we know for any $w_1\in (\frac{1}{2},\frac{1}{2}+\delta)$, there exists $\theta_w\in (-\theta^*,\theta_0)$ and an $\epsilon$-neighborhood of $\theta_w$ such that 
%\begin{eqnarray}
%H(\theta;\theta^*,w_1)-\theta&>&0, \quad \quad \forall \theta\in (\theta_w-\epsilon,\theta_w)\n\\
%H(\theta_w;\theta^*,w_1)-\theta_w&=&0,\n\\
%H(\theta;\theta^*,w_1)-\theta&<&0, \quad \quad \forall \theta\in (\theta_w,\theta_w+\epsilon).\n
%\end{eqnarray} 
%Therefore, $\theta_w$ is a stable fixed point in $(-\theta^*,0)$ for a given $w_1\in (\frac{1}{2},\frac{1}{2}+\delta)$.









  

